ADOPT: Adaptively Optimizing Attribute Orders for Worst-Case Optimal Join Algorithms via Reinforcement Learning

The performance of worst-case optimal join algorithms depends on the order in which the join attributes are processed. Selecting good orders before query execution is hard, due to the large space of possible orders and unreliable execution cost estimates in case of data skew or data correlation. We propose ADOPT, a query engine that combines adaptive query processing with a worst-case optimal join algorithm, which uses an order on the join attributes instead of a join order on relations. ADOPT divides query execution into episodes in which different attribute orders are tried. Based on run time feedback on attribute order performance, ADOPT converges quickly to near-optimal orders. It avoids redundant work across different orders via a novel data structure, keeping track of parts of the join input that have been successfully processed. It selects attribute orders to try via reinforcement learning, balancing the need for exploring new orders with the desire to exploit promising orders. In experiments with various data sets and queries, it outperforms baselines, including commercial and open-source systems using worst-case optimal join algorithms, whenever queries become complex and therefore difficult to optimize.

==> sections/model.tex <==
\section{Problem Model}

We introduce our problem model, related terminology and notations. We consider the following type of queries ... (TODO). 

ADOPT uses the leapfrog triejoin, a worst-case optimal join algorithm, as basis. This algorithm operates on combinations of join attribute values. The set of all possible combinations can be represented as a multi-dimensional cube. By the term ``cube'', we generally refer to cubes of join attribute values in the following. Given a cube $c$, we denote by $c.l$ and $c.u$ the vector of lower and upper cube bounds respectively. Furthermore, we use the subscript to refer to bounds in specific dimensions (e.g., $c.l_i$ refers to the lower bound for the $i$-th attribute within cube $c$). 

TODO: what else should we introduce here?

==> sections/questions.tex <==
Is there any prior work on the performance impact of different variable orders on worst-case optimal join algorithms?

Is there any prior work on worst-case optimal algorithms that do not depend on a variable order (following~\cite{Navarro2019})?

Possibilities to include non-intrusive versions of the learning approach into LogicBlox?

==> sections/related.tex <==

% Claim that their worst-case optimal join algorithm does not depend on an attribute order, the complexity contains however a few factors that grow quickly in the query size ~\cite{Navarro2019}.

% Factorized databases~\cite{Olteanu2016}. 



==> sections/reward.tex <==
\begin{algorithm}[t!]
\caption{}
\label{alg:rl_wcj}
\renewcommand{\algorithmiccomment}[1]{// #1}
\begin{small}
\begin{algorithmic}[1]
\State \textbf{Input:} SPJ query $q$, budget of each episode $b$
\State \textbf{Output:} Result $r$
\Function{RL\_WCJ}{$q, b$}
\State $q \gets$ \Call{ApplyUnaryPredicates}{$q$}
\State $q \gets$ \Call{DistinctJoinValues}{$q$}
\State $finish \gets true$ 
\While {$\lnot finish$}
\State \Comment{Retrieve an attribute order to evaluate}
\State $o \gets$ \Call{MCTSSample}{q}
\State \Comment{Restore execution state for this join order}
\State $s \gets$ \Call{RestoreState}{$o$}
\State \Comment{Execute join order during time budget}
\State $finish, rw \gets$ \Call{ContinueJoin}{s, o, b}
\State \Call{RewardUpdate}{$rw$}
\EndWhile
\EndFunction
\end{algorithmic}
\end{small}
\end{algorithm}

\begin{algorithm}[t!]
\caption{}
\label{alg:rl_wcj}
\renewcommand{\algorithmiccomment}[1]{// #1}
\begin{small}
\begin{algorithmic}[1]
\State \textbf{Input:} State $s$, attribute order $o$ and budget $b$
\State \textbf{Output:} Reward $rw$
\Function{ContinueJoin}{$s, o, b$}
\State \Comment{$s.tuplevalue$ include keys to seek for each attribute}
\State \Comment{$s.l$ is the length of shared prefix}
\State $stv \gets s.tuplevalue$
\If{$s.l == o.len$}
\State \Comment{Continue from the last position}
\State \Call{LFTJ}{}
\Else
\State \Comment{Change the position of iterators}
    \State \Comment{Reset all iterators to the begining}
    \For{$it \in iters$}
    \State \Call{Reset}{$it$}
    \EndFor
    \For{$i\gets0,\ldots,s.l$}
    \State \Comment{Get the seek value for $i$-th attribute}
    \State $k \gets stv[i]$
    \For{$it \in iters[i]$}
    \State \Comment{Get each iterator for i-th attribute}
    \State \Call{it.open}{ }
    \State \Call{it.seek}{k}
    \EndFor
    \EndFor
    \State $vid \gets s.l$
    \State \Call{LFTJ}{$vid$}
\State
\EndIf 
\EndFunction
\end{algorithmic}
\end{small}
\end{algorithm}



\begin{algorithm}[t!]
\caption{}
\label{alg:rl_wcj}
\renewcommand{\algorithmiccomment}[1]{// #1}
\begin{small}
\begin{algorithmic}[1]
\State \textbf{Input:} State $s$, attribute order $o$ and budget $b$
\State \textbf{Output:} Reward $rw$
\Function{ContinueJoin}{$s, o, b$}
\State \Comment{$s.tuplevalue$ include keys to seek for each attribute}
\State \Comment{$s.l$ is the length of shared prefix}
\State $stv \gets s.tuplevalue$
\If{$s.l == o.len$}
\State \Comment{Continue from the last position}
\State \Call{LFTJ}{}
\Else
\State \Comment{Change the position of iterators}
    \State \Comment{Reset all iterators to the begining}
    \For{$it \in iters$}
    \State \Call{Reset}{$it$}
    \EndFor
    \For{$i\gets0,\ldots,s.l$}
    \State \Comment{Get the seek value for $i$-th attribute}
    \State $k \gets stv[i]$
    \For{$it \in iters[i]$}
    \State \Comment{Get each iterator for i-th attribute}
    \State \Call{it.open}{ }
    \State \Call{it.seek}{k}
    \EndFor
    \EndFor
    \State $vid \gets s.l$
    \State \Call{LFTJ}{$vid$}
\State
\EndIf 
\EndFunction
\end{algorithmic}
\end{small}
\end{algorithm}
